Search for W' boson production in the W'->tb decay channel

We present a search for the production of a new heavy gauge boson W' that decays to a top quark and a bottom quark. We have analyzed 230 pb^{-1} of data collected with the Dzero detector at the Fermilab Tevatron collider at a center-of-mass energy of 1.96 TeV. No significant excess of events above the standard model expectation is found in any region of the final state invariant mass distribution. We set upper limits on the production cross section of W' bosons times branching ratio to top quarks at the 95% confidence level for several different W' boson masses. We exclude masses between 200 GeV and 610 GeV for a W' boson with standard-model-like couplings, between 200 GeV and 630 GeV for a W' boson with right-handed couplings that is allowed to decay to both leptons and quarks, and between 200 GeV and 670 GeV for a W' boson with right-handed couplings that is only allowed to decay to quarks.

==> list_of_visitor_addresses_r2.tex <==
% list_of_visitor_addresses_r2.tex                            6/19/06
%
\bibitem[*]{kurca}
On leave from IEP SAS Kosice, Slovakia.
\bibitem[\dag]{voutilainen}
Visitor from Helsinki Institute of Physics, Helsinki, Finland.
\bibitem[\ddag]{kozminski}
Visitor from Lewis University, Romeoville, IL, USA
%
\vskip 0.25cm

